Improving Passage Retrieval with Zero-Shot Question Generation

We propose a simple and effective re-ranking method for improving passage retrieval in open question answering. The re-ranker re-scores retrieved passages with a zero-shot question generation model, which uses a pre-trained language model to compute the probability of the input question conditioned on a retrieved passage. This approach can be applied on top of any retrieval method (e.g. neural or keyword-based), does not require any domain- or task-specific training (and therefore is expected to generalize better to data distribution shifts), and provides rich cross-attention between query and passage (i.e. it must explain every token in the question). When evaluated on a number of open-domain retrieval datasets, our re-ranker improves strong unsupervised retrieval models by 6%-18% absolute and strong supervised models by up to 12% in terms of top-20 passage retrieval accuracy. We also obtain new state-of-the-art results on full open-domain question answering by simply adding the new re-ranker to existing models with no further changes.

==> table/tab-rerank-algo-cmp.tex <==
% !TeX root = ../main.tex
% !TeX spellcheck


\begin{table*}[!ht]
\small
\centering
\begin{tabular}{l l | c c c c | c c c c}
 \toprule
 \tf{Re-Ranker PLM} & \tf{Retriever} & \multicolumn{4}{c}{\tf{TriviaQA (dev.\ set)}} & \multicolumn{4}{c}{\tf{NQ (dev.\ set)}}  \\
                    &           &  Top-1 & Top-5 & Top-20 & Top-100 & Top-1 & Top-5 & Top-20 & Top-100 \\
\midrule
% \multicolumn{10}{c}{Before Re-Ranking} \\
% \midrule
       & BM25                   &   46.5 &  66.4 &  76.6  &  83.0   & 22.3  & 43.8  & 62.3   &  76.0  \\  
       & MSS                    &   30.2 &  52.0 &  67.1  &  79.4   & 17.7  & 38.6  & 57.4   &  72.4 \\
% \midrule
% \multicolumn{10}{c}{After Re-Ranking} \\
% \midrule
GPT-neo (2.7B)  & BM25 + MSS    &   52.3 &  74.3 &  82.6  &  86.9   & 27.2  & 55.0  & 73.9   &  84.2 \\
T5-xl (3B)  & BM25 + MSS        &   45.0 &  70.4 &  81.3  &  86.4   & 22.0  & 50.5  & 71.4   &  84.0 \\
T5-xl-lm-adapt (3B) & BM25 + MSS&   53.1 &  75.3 &  83.4  &  87.1   & 29.7  & 59.9  & 76.9   & 85.6 \\
T0-3B  & BM25 + MSS             & \tf{58.2} & \tf{77.8} & \tf{86.3} & \tf{87.4} & \tf{36.7} & \tf{64.9} & \tf{79.1} & \tf{86.1} \\

\bottomrule
\end{tabular}
\caption{Effect of using different pre-trained language models (PLMs) as rerankers. Top-\{1, 5, 20, 100\} retrieval accuracy on the development set of datasets before and after performing unsupervised re-ranking of the top-2000 retrieved documents. Please see text for the description of different pre-trained language models.}
\label{tab:qa-reranking-plms}
\end{table*}


